Answering Product-Questions by Utilizing Questions from Other Contextually Similar Products

Predicting the answer to a product-related question is an emerging field of research that recently attracted a lot of attention. Answering subjective and opinion-based questions is most challenging due to the dependency on customer-generated content. Previous works mostly focused on review-aware answer prediction; however, these approaches fail for new or unpopular products, having no (or only a few) reviews at hand. In this work, we propose a novel and complementary approach for predicting the answer for such questions, based on the answers for similar questions asked on similar products. We measure the contextual similarity between products based on the answers they provide for the same question. A mixture-of-expert framework is used to predict the answer by aggregating the answers from contextually similar products. Empirical results demonstrate that our model outperforms strong baselines on some segments of questions, namely those that have roughly ten or more similar resolved questions in the corpus. We additionally publish two large-scale datasets used in this work, one is of similar product question pairs, and the second is of product question-answer pairs.

==> Figs/pqa_stats_av.tex <==

\begin{tabular}{ccccc}                                                                 
    \toprule                                                                                   
         & \textbf{Train} &  \textbf{Dev} & \textbf{Test} & \textbf{Total}\\
    \midrule                                                                                   
	\textbf{\# Products}		&     55,006 	&  6,872 	&  6,872 	&  68,750 \\
	\textbf{\# Questions}		&    201,403 	&  23,859 	&  26,260 	&  251,522 \\
	\textbf{\% Yes}	        &      66.5\%	& 66.0\%	& 66.0\%	& 66.4\%*\\
    \bottomrule                                                                                
                                                                                               
\end{tabular}                                                                                  
                                                                                               


==> Figs/prep_dataset.tex <==

\begin{tabular}{p{2.6cm}cccc}
    \toprule
    \textbf{} & \textbf{Column1} &  \textbf{Column2} & \textbf{Column3} \\
    \midrule
%    \rowcolor{lightgray} \multicolumn{5}{c}{Criteria} \\ 
%    \midrule
%    \textbf{Depth* } & 1 - 3 & 4 - 6 & $> 7$ \\
%    \textbf{Length} & 6 - 15 & 16 - 25 & $>26$ \\
    \rowcolor{lightgray} \multicolumn{4}{c}{placeholder 1} \\ 
    \textbf{Light Bars        } & 10 & 9 & 28 \\
    \textbf{Monitors          } & 10 & 9 & 28 \\
    \textbf{Smartwatches      } & 10 & 9 & 28 \\
    \textbf{Receivers         } & 10 & 9 & 28 \\
    \textbf{Backpacks         } & 10 & 9 & 28 \\
    \textbf{Jeans             } & 10 & 9 & 28 \\
    \textbf{Beds              } & 10 & 9 & 28 \\
    \textbf{Home Office Desks } & 10 & 9 & 28 \\
    \textbf{Masks             } & 10 & 9 & 28 \\
    \textbf{Posters \& Prints } & 10 & 9 & 28 \\
    \textbf{Accessories       } & 10 & 9 & 28 \\
    \rowcolor{lightgray} \multicolumn{4}{c}{placeholder 1} \\ 
    \textbf{row12} & 21K  & 34K & 91K  \\
    \textbf{row13} & 181K & 182K & 602K  \\    
    \bottomrule
\end{tabular}





==> myRelated.tex <==

\begin{comment}
\cite{DBLP:conf/www/McAuleyY16}
In this paper we hope to fuse these two paradigms: given a large volume of previously answered queries about products, we hope to automatically learn whether a review of a product is relevant to a given query. We formulate this as a machine learning problem using a mixture-of-experts-type framework---here each review is an `expert' that gets to vote on the response to a particular query; simultaneously we learn a relevance function such that `relevant' reviews are those that vote correctly.

\cite{wan2016modeling}
While recent work introduced the idea of question-answering using product reviews, it did not account for two aspects that we consider in this paper: (1) Questions have multiple, often divergent, answers, and this full spectrum of answers should somehow be used to train the system, and (2) What makes a 'good' answer depends on the asker and the answerer, and these factors should be incorporated in order for the system to be more personalized.

\cite{Deng2020}
In this paper, we tackle opinion-aware answer generation by jointly learning answer generation and opinion mining tasks with a unified model. Two kinds of opinion fusion strategies, namely, static and dynamic fusion, are
proposed to distill and aggregate important opinion information learned from the opinion mining task into the answer generation process.

\cite{DBLP:conf/wsdm/GaoRZZYY19}
In this paper, we propose the task of product-aware answer generation, which tends to generate an accurate and complete answer from large-scale unlabeled e-commerce reviews and product attributes. we propose an adversarial learning based model, named PAAG, which is composed of three components: a question-aware review representation module, a key-value memory network encoding attributes, and a recurrent neural network as a sequence generator.

\cite{chen2019answer}
In this paper, we investigate how to provide a quick response to the asker by plausible answer identification from product reviews. By analyzing the similarity and discrepancy between explicit answers and reviews
that can be answers, a novel multi-task deep learning
method with carefully designed attention mechanisms is developed. The method can well exploit large amounts of user generated QA data and a few manually labeled review data to address the problem.

\cite{DBLP:conf/wsdm/YuL18}
Both Question Answering (QA) approaches and Community Question Answering methods are not suitable for answer prediction for new questions in this setting. The reasons are that questions are product-associated and many of them are concerned about user experiences and subjective opinions. In this paper, we propose a new framework that can tackle the task of review-aware answer prediction for product-related questions. The aspect analytics model in this framework learns latent aspects as well as aspect-specific embeddings of reviews via a 3-order Autoencoder. One advantage of this learned model is that it can generate aspect-specific representations for new questions. The predictive answer model in our framework, learned jointly from existing questions, answers, and reviews, is able to predict the answers for new yes-no questions taking into consideration of aspects. 


\cite{Yu2018}
A key solution to these QA systems is to retrieve from a QA knowledge base the most similar question of a given question, which can be reformulated as a paraphrase identification (PI) or a natural language inference (NLI) problem. In this paper, we study transfer learning for the PI and NLI problems, aiming to propose a general framework, which can effectively and efficiently adapt the shared knowledge learned from a resource-rich source domain to a resource-poor target domain. Specifically, since most existing transfer learning methods only focus on learning a shared feature space across domains while ignoring the relationship between the source and target domains, we propose to simultaneously learn shared representations and domain relationships in a unified framework. Furthermore, we propose an efficient and effective hybrid model by combining a sentence encoding-based method and a sentence interaction-based method as our base model.

\cite{yu2012answering}
This paper proposes to generate appropriate
answers for opinion questions about products by exploiting the hierarchical organization of consumer reviews. The hierarchy organizes product aspects as nodes following their parent-child relations. For each aspect, the reviews and corresponding opinions on this aspect are stored. We develop a new framework
for opinion Questions Answering, which enables accurate question analysis and effective answer generation by making use the hierarchy. In particular, we first identify the (explicit/implicit) product aspects asked in the questions and their sub-aspects by referring
to the hierarchy. We then retrieve the corresponding review fragments relevant to the aspects from the hierarchy. In order to generate appropriate answers from the review fragments, we develop a multi-criteria optimization approach for answer generation by simultaneously taking into account review salience,
coherence, diversity, and parent-child relations among the aspects.

\cite{Zhao2019}
Most recent PQA approaches adopt end2end semantic matching methodologies, which map questions and answers to a latent vector space to measure their relevance. Such methods often achieve superior performance but it tends to be difficult to interpret why. On the other hand, simple keyword-based search methods exhibit natural interpretability through matched keywords, but often suffer from the lexical gap problem. In this work, we develop a new PQA framework (named Riker) that enjoys the benefits of both interpretability and effectiveness. Riker mines rich keyword representations of a question with two major components, internal word re-weighting and external word association, which predict the importance of each question word and associate the question with outside relevant keywords respectively, and can be jointly trained under weak supervision with large-scale QA pairs. The keyword representations from Riker can be directly used as input to a keyword-based search module, enabling the whole process to be effective while preserving good interpretability.

\cite{fan2019reading}
The mainstream approaches on PQA generally employ customer reviews as the evidence to help predict answers to the questions which are product-specific and concerned more about subjective personal experiences. However, the supportive features either extracted by heuristic rules or acquired from unsupervised manners are not able to perform well on PQA. In this paper, we contribute an end-to-end neural architecture directly fed by the raw text of product-related questions and customer reviews to predict the answers. Concretely, it teaches machines to generate and to synthesize multiple question-aware review representations in a reading comprehension fashion to make the final decision.

\cite{Zhang2019}
Previous research suggests that reviews are a valuable resource for answering product queries, but a key challenge is the language mismatch between user queries and reviews. To address this, we propose two neural models that discover relevant reviews for answering product queries. We demonstrate that our best model produces strong performance, outperforming state-of-the-art systems by consistently finding the most relevant reviews for product queries.

\cite{ddas2019learning}
In this work, we explore several recently successful neural approaches to modeling sentence pairs, that could better learn the relationship between questions and ground truth answers, and thus help infer reviews that can best answer a question or augment a given answer. In particular, we hypothesize that our adversarial domain adaptation-based approach, due to its ability to additionally learn domain-invariant features from a large number of unlabeled, unpaired question-review samples, would perform better than our proposed baselines, at answering specific, subjective product-related queries using reviews.

\cite{Lai2018}
In this paper, we show that the large volume of existing community question answering data can be beneficial when building a system for answering questions related to product facts and specifications. Our experimental results demonstrate that the performance of a model for answering questions related to products listed in the Home Depot website can be improved by a large margin via a simple transfer learning technique from an existing large-scale Amazon community question answering dataset.

\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

